NOPE: Novel Object Pose Estimation from a Single Image

The practicality of 3D object pose estimation remains limited for many applications due to the need for prior knowledge of a 3D model and a training period for new objects. To address this limitation, we propose an approach that takes a single image of a new object as input and predicts the relative pose of this object in new images without prior knowledge of the object's 3D model and without requiring training time for new objects and categories. We achieve this by training a model to directly predict discriminative embeddings for viewpoints surrounding the object. This prediction is done using a simple U-Net architecture with attention and conditioned on the desired pose, which yields extremely fast inference. We compare our approach to state-of-the-art methods and show it outperforms them both in terms of accuracy and robustness. Our source code is publicly available at https://github.com/nv-nguyen/nope

==> sections/1_intro.tex <==
Estimating the 3D pose of objects has seen significant progress in the past decade with regard to both robustness and accuracy~\cite{kehl-iccv17-ssd6d,rad-iccv17-bb8,tekin-cvpr18-realtimeseamlesssingleshot,li-eccv18-deepim,zakharov-iccv19-dpod}. Specifically, there has been a considerable increase in robustness to partial occlusions~\cite{peng-cvpr19-pvnet,hu-cvpr19-segmentationdriven6dobjectposeestimation,oberweger-eccv18-makingdeepheatmapsrobust}, and the need for large amounts of real annotated training images has been relaxed through the use of domain transfer~\cite{baek-cvpr20-weaklysuperviseddomainadaptation}, domain randomization~\cite{tremblay-18-deepobjectposeestimation,loing-ijcv18-virtual,labbe-eccv20-cosypose,sundermeyer-cvpr20-multipathlearning}, and self-supervised learning techniques~\cite{sundermeyer-ijcv20-augmentedautoencoders} that leverage synthetic images for training.

Unfortunately, the practicality of 3D object pose estimation remains limited for many applications, including robotics and augmented reality. Typically, existing approaches require a 3D model~\cite{megapose,nguyen2022templates,nguyen2024gigaPose}, a video sequence~\cite{onepose,oneposepp}, or sparse multiple images of the target object~\cite{relpose}, and a training stage. Several techniques aim to prevent the need for retraining by assuming that new objects fall into a recognized category~\cite{Grabner_CVPR18,Wang_2019_NOCS}, share similarities with the previously trained examples as in the T-LESS dataset~\cite{sundermeyer-cvpr20-multipathlearning}, or exhibit noticeable corners~\cite{Pitteri20203DOD}.



In this paper, we introduce an approach, which we call {\bf NOPE} for {\bf N}ovel {\bf O}bject {\bf P}ose {\bf E}stimation, that only requires a single image of the new object to predict the relative pose of this object in any new images, without 
the need for the object's 3D model and without training on the new object.
This is a very challenging task, as, by contrast with the multiple views used in \cite{onepose,relpose} for example, a single view only provides limited information about the object's geometry.



To achieve this, we train NOPE to generate novel views of an object. These novel views can be used as `templates' annotated with the corresponding poses.  Matching these templates with new input views lets us estimate the object relative pose with respect to the initial view. Our approach relates to the recent development in novel view synthesis. However, we take this one step further: Motivated by the good performance of recent template matching work for pose estimation~\cite{nguyen2022templates, shugurov_osop_2022}, instead of predicting plain color images, we directly predict discriminative embeddings of the views. These embeddings are extracted by passing the input image through a U-Net architecture with attention and conditioned on the desired pose for the new view.


In essence, in contrast to existing novel view synthesis works~\cite{realfusion, poole2022dreamfusion}, for our pose estimation task, we do not need to create a 3D model of the object. This saves significant computation time, as optimizing a 3D model using a single view takes at least one hour~\cite{sparsefusion} or longer~\cite{neuralLift}. 
By contrast, our approach based on direct inference of the view embeddings is extremely fast, processing an image in less than 2 seconds. Yet, it yields accurate pose estimates with more than 59 accuracy on average on unseen instances or categories. Our work is also related to motion prediction between 2 images, such as~\cite{ummenhofer-cvpr17-demon,nguyen_pizza_2022}, which predict the camera displacement between two images. Our comparisons to the closest work to ours~\cite{nguyen_pizza_2022} show that we significantly outperform this approach.


Furthermore, we show that our approach can identify the pose ambiguities due, for example, to symmetries~\cite{tombari}, even if we do not have access to the object 3D model but only to a single view.
To this end, we estimate the distribution over all poses for the query, which becomes increasingly less peaked as the pose suffers from increasingly many ambiguities. Figure~\ref{fig:teaser} depicts a variety of ambiguous and unambiguous cases with their pose distributions.


In summary, our main contribution is to show that we can  efficiently and reliably recover the relative pose of an unseen object in novel views given only a single view of that object. To the best of our knowledge, our approach is the first to predict ambiguities due to symmetries and partial occlusions of unseen objects from only a single view.

==> sections/3_method.tex <==
\vspace{-6pt}
In this section, we first motivate our approach with an experiment based on novel view generation.
We then describe our architecture, how we train it, and how we use it for pose prediction and for identifying pose ambiguities.

\input{sections/3a_motivation}

\input{sections/3_main_figure.tex}

\label{sec:motivation}

\subsection{Framework}
\label{sec:framework}
Figure~\ref{fig:framework} gives an overview of our approach. 
We train a deep architecture to generate embeddings of novel views of an object using pairs of images of objects from a first set of object categories. In practice, we consider embeddings computed from the pretrained VAE of~\cite{stable-diffusion}, as it was shown to yield a robust representation for template matching. To generate these embeddings, we use a U-Net-like network with a pose conditioning mechanism that is very close to the one introduced in 3DiM~\cite{3dim} and related to the text-to-image mechanism in \cite{stable-diffusion}. 

More precisely, we first use a Multilayer Perceptron~(MLP) to convert the desired relative viewpoint $\Delta R$ with respect to the object pose in the reference view to a pose embedding. We then integrate this pose embedding into the feature map at every stage of our U-Net using cross-attention, as described in \cite{stable-diffusion}. 

\vspace*{-15pt}
\paragraph{Training.} At each iteration, we build a batch composed of $N$ pairs of images, a reference image and another image of the same object with a known relative pose. The U-Net model takes as input the embedding of the reference image and as conditioning the embedding of the relative pose to predict an embedding for the second image. We jointly optimize the U-Net and the MLP by minimizing the Euclidean distance between this predicted embedding and the embedding of the query image. \nguyen{Note that we freeze the pretrained VAE network of \cite{stable-diffusion} during the training.}

By training it on a diverse dataset of objects, this architecture generalizes well to  novel unseen object categories. \nguyen{Interestingly, our method does not explicitly learn any symmetries during training, but it is able to detect pose ambiguities during testing as discussed below.}


\subsection{Pose prediction}
\label{sec:templateMatching}

\vspace{-4pt}
\paragraph{Template matching.} 
Once our architecture is trained, we can use it to generate the embeddings for novel views: Given a reference image $\imageRef$ and a set of $N$ relative viewpoints $\mathcal{P}=\left(\relativeR_1, \relativeR_2, \dots, \relativeR_N \right)$, we can obtain a corresponding set of predicted embeddings $(\mathbf{e}_1, \mathbf{e}_2, \dots, \mathbf{e}_N)$. To define these viewpoints, we follow the approach used in \cite{nguyen2022templates}: We start with a regular icosahedron and subdivide each triangle recursively into four smaller triangles twice to get 342 final viewpoints. Finally, we simply perform a nearest neighbor search to determine the reference point that has the embedding closest to the embedding of the query image. 
%Note that this can be done efficiently~\cite{nguyen2022templates}.

\vspace{-8pt}
\paragraph{Detecting pose ambiguities.} Pose ambiguities arise when the object has symmetries or when an object part that could remove the ambiguity is not visible, as for the mug in Figure~\ref{fig:teaser}. By considering the distance between the embedding of the query image and the generated embeddings, we not only can predict a single pose but also identify all the other poses that are possible given the reference and query views.

\newcommand{\be}{{\bf e}}

More formally, we estimate the probability of a relative pose $\Delta R$ given reference image $I_r$ and query image $I_q$ as
%
\begin{equation}
p(\Delta R \; | \; I_r, I_q) = \frac{1}{Z} \frac{\be_{\Delta R} \cdot \be_q}{\| \be_{\Delta R} \| \| \be_q \|} \> ,
\end{equation}
%
where $\be_{\Delta R}$ is the embedding predicted by the U-Net from reference image $I_r$ and relative pose $\Delta R$, $\be_q$ is the embedding for query image $I_q$, and $Z$ is a normalization factor. The operator $\cdot$ denotes the dot product.

\input{sections/3_symmetry}

To illustrate this, we show in Figure~\ref{fig:symmetry} three distinct types of symmetry and visualize the pose distribution for corresponding pairs of  reference and query images~(not shown). The number of regions with high similarity scores is consistent with the number of symmetries and pose ambiguities:  If an object has no symmetry, the probability distribution has a clear mode. The probability distribution for objects with symmetries have typically several modes or even a continuous high-probability region in case of rotational symmetry. We provide additional qualitative results in Section~\ref{sec:experiments}.



==> sections/3_reconstruction.tex <==
\begin{figure}[t]
\newlength{\plotheight}
\setlength\plotheight{1.9cm}
\centering
\setlength\lineskip{2.5pt}
\setlength\tabcolsep{2.5pt} 
{\small
\begin{tabular}{
% 
>{\centering\arraybackslash}m{\plotheight}
>{\centering\arraybackslash}m{\plotheight}%|
>{\centering\arraybackslash}m{\plotheight}%|
>{\centering\arraybackslash}m{\plotheight}
}

Reference & GT & 3DiM \cite{3dim} & Our method \\
\frame{\includegraphics[height=\plotheight, ]{figures/method/ref.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/gt.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/3dim.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/ours.png}}\\[0em]
%\hline
\frame{\includegraphics[height=\plotheight, ]{figures/method/ref2.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/gt2.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/3dim2.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/ours2.png}}\\
\end{tabular}
}
\vspace{-4mm}
\caption{\nguyen{{\bf View Synthesis vs Pose Estimation.} While there is a connection between view synthesis and 3D pose estimation, there is no direct correlation between them. In fact, despite 3DiM \cite{3dim} producing better overall view synthesis in pixel level, it demonstrates lower performance in 3D object pose estimation compared to our method when used for this task. }
\vincentrmk{I dont understand what are the images and what you want to show here.  
What I understand is that the images for our method are generated using stable diffusion from our predicted embeddings, but what does it show?
}
}\nguyenrmk{Sorry, let's remove this figure, it's not helpful. What I want to show with this figure is that there is no correlation between view synthesis in pixel space and  3D pose estimation template matching. Indeed, through our experiments, we found that 3DiM always have good results on view synthesis in pixel space but not very good in pose estimation. This observation motivates us to skip view synthesis in pixel space but focus on feature space since we can use discriminate features which is proven in \cite{nguyen_templates_2022} more helpful for 3d object pose estimation}
\label{fig:reconstruction}
\end{figure}

==> sections/3a_motivation.tex <==
\vspace{-4pt}
\subsection{Motivation}
\vspace{-4pt}
To motivate our approach, we evaluate the use of the state-of-the-art 3D model-based image generation method (3DiM)~\cite{3dim} for pose estimation. 3DiM is a diffusion-based method for view synthesis in pixel space. To apply it to pose prediction given a reference image of an object, we experimented with using it to generate a set of novel views from many different viewpoints and match a query image of the object to these views in pixel space. Since the generated views are annotated with the corresponding pose, this gives us a pose estimate. 

As shown in Figure~\ref{fig:motivation}, the images generated by 3DiM look very realistic. However, the recovered poses are not very accurate. This can be explained in part by the fact that diffusion can ``invent'' details that disturb image matching. The limitations of this approach will further be quantitatively demonstrated in our experiments (Table~\ref{tab:shapeNet}). This motivates us to learn to directly generate a discriminative representation of the views.


\begin{figure}[t]
\newlength{\plotheight}
\setlength\plotheight{1.5cm}
\centering
\setlength\lineskip{2.0pt}
\setlength\tabcolsep{2.0pt} 
{\small
\begin{tabular}{
% 
>{\centering\arraybackslash}m{\plotheight}
>{\centering\arraybackslash}m{\plotheight}
>{\centering\arraybackslash}m{\plotheight}%|
>{\centering\arraybackslash}m{\plotheight}%|
>{\centering\arraybackslash}m{\plotheight}
}
 & & Generated & Recovered &  \\
 & & view from & pose by & Estimated \\
 & & the query & template &  pose \\
Reference & Query & GT pose & matching & distribution \\
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample3/ref.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample3/query.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample3/3dim.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample3/pose.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample1/proba.png}}\\[0em]
%\hline
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample4/ref.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample4/query.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample4/3dim.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample4/pose.png}}&
\frame{\includegraphics[height=\plotheight, ]{figures/method/motivation/sample2/proba.png}}\\
\end{tabular}
\begin{tabular}{
>{\centering\arraybackslash}m{0.3\teaserheight}
}
\includegraphics[height=3\teaserheight, ]{figures/teaser/colorbar.png}\\
\end{tabular}
}
\vspace*{-20pt}
\caption{
\textbf{The limit of image generation with diffusion models for pose prediction.} While the images generated by 3DiM look very realistic, they may change the appearance of the object, impairing the similarity computation between the query image and the generated view, and hence the pose estimation when used for our problem. Notice that the probability distributions does not peak on the right pose but shows many wrong local maxima.
}
\label{fig:motivation}
\end{figure}

% \vincentrmk{I dont understand what are the images and what you want to show here.  
% What I understand is that the images for our method are generated using stable diffusion from our predicted embeddings, but what does it show?
% }

==> sections/4_occluded_test_sets.tex <==
\begin{figure}[t]
% \newlength{\plotHeight}
\setlength\plotHeight{1.8cm}
\centering
\setlength\lineskip{1.5pt}
\setlength\tabcolsep{1.5pt} 
{\footnotesize
\begin{tabular}{c}
\begin{tabular}{
>{\centering\arraybackslash}m{\plotHeight}
>{\centering\arraybackslash}m{\plotHeight}
>{\centering\arraybackslash}m{\plotHeight}
>{\centering\arraybackslash}m{\plotHeight}
}
\frame{\includegraphics[width=\plotHeight, ]{figures/experiments/occlusions/bottle.png}}&
\frame{\includegraphics[width=\plotHeight, ]{figures/experiments/occlusions/cup.png}}&
\frame{\includegraphics[width=\plotHeight, ]{figures/experiments/occlusions/dishwasher.png}}&
\frame{\includegraphics[width=\plotHeight, ]{figures/experiments/occlusions/train.png}}\\

\end{tabular}

% \begin{tabular}{@{\;\;\;\;}
% >{\arraybackslash}m{5cm}
% }
% \includegraphics[height=0.35\teaserheight, ]{figures/teaser/colorbar.png}\\
% \end{tabular}\\

\end{tabular}}
\caption{\nguyen{{\bf Samples of occluded test sets.} We use Random Erasing \cite{zhong2020random} to generate occlusions on objects for testing robustness of our methods to occlusions. }}
\label{fig:occlusionSamples}
\end{figure} 

==> sections/4_qualitative_v0.tex <==
\begin{figure*}
\newlength{\imageheight}
\setlength\imageheight{1.5cm}
\centering
\setlength\lineskip{1.pt}
\setlength\tabcolsep{1.pt} 
{\small
\begin{tabular}{c}
\begin{tabular}{
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
\hline
\multicolumn{11}{c}{\textbf{without occlusions}}\\
\hline
\\[-0.2cm]
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_2_10_10/4_ref_2_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_2_10_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_2_10_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_2_10_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_2_10_10/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_6_14_1/4_ref_2_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_6_14_1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_6_14_1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_6_14_1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bottle_6_14_1/proba2.png}}\\

% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_85_50_5/0_pred_crop.png}} &
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_85_50_5/1_query_crop.png}} &
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_85_50_5/pizza.png}}&
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_85_50_5/0_pred_crop.png}}&
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_85_50_5/proba.png}}&
% &
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_104_68_15/3_ref_1_crop.png}} &
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_104_68_15/1_query_crop.png}} &
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_104_68_15/pizza.png}}&
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_104_68_15/0_pred_crop.png}}&
% \frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/bus_104_68_15/proba.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_138_31_9/0_pred_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_138_31_9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_138_31_9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_138_31_9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_138_31_9/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_159_50_6/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_159_50_6/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_159_50_6/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_159_50_6/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/clock_159_50_6/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_8/0_pred_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_8/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_10/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/dishwasher_167_3_10/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_189_24_0/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_189_24_0/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_189_24_0/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_189_24_0/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_189_24_0/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_193_28_15/3_ref_1_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_193_28_15/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_193_28_15/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_193_28_15/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/guitar_193_28_15/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug2/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug2/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug2/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug2/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug2/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug11/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug11/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug11/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug11/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/mug11/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol1/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol1/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol9/4_ref_2_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/pistol9/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard1/3_ref_1_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard1/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard13/4_ref_2_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard13/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard13/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard13/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/skateboard13/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train1/3_ref_1_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train1/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train7/4_ref_2_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train7/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train7/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train7/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/train7/proba2.png}}\\[0.1cm]


\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer0/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer0/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer0/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer0/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer0/proba2.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer8/2_ref_0_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative/washer8/proba2.png}}\\

\hline
\multicolumn{11}{c}{\textbf{with partial occlusions}}\\
\hline
\\[-0.2cm]


\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bus_66_33_0/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bus_66_33_0/query.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bus_66_33_0/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bus_66_33_0/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bus_66_33_0/proba2.png}}&
&

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/dishwasher_165_1_1/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/dishwasher_165_1_1/query.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/dishwasher_165_1_1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/dishwasher_165_1_1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/dishwasher_165_1_1/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_124_19_11/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_124_19_11/query.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_124_19_11/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_124_19_11/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_124_19_11/proba2.png}}&
&

\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_142_35_7/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_142_35_7/query.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_142_35_7/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_142_35_7/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/clock_142_35_7/proba2.png}}\\

\frame{\includegraphics[height=\imageheight, ]{figures/teaser/bottle_4_12_0/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/teaser/bottle_4_12_0/query.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/teaser/bottle_4_12_0/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/teaser/bottle_4_12_0/pred.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/teaser/bottle_4_12_0/proba2.png}}&

&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bottle_0_0_5/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bottle_0_0_5/query.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bottle_0_0_5/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bottle_0_0_5/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/experiments/qualitative_occlusion/bottle_0_0_5/proba2.png}}\\

Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution & &Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution\\
\end{tabular}
\end{tabular}
}
\vspace{-3mm}
\caption{\label{fig:qualitative} {\bf Visual results on unseen categories} from ShapeNet. An arrow indicates the pose with the highest probability as recovered by our method. We visually compare with PIZZA, which is the method with the second best performance. \textbf{We visualize the predicted poses by rendering the object from these poses, but the 3D model is only used for visualization purposes, not as input to our method. Similarly, we use the canonical pose of the 3D model to visualize this distribution, but not as input to our method.}
} 
\end{figure*}

==> sections/6_supp_qualitative.tex <==
\begin{figure*}
\newlength{\imageheight}
\setlength\imageheight{1.50cm}
\centering
\setlength\lineskip{3.pt}
\setlength\tabcolsep{2.pt} 
{\small
\begin{tabular}{c}
\begin{tabular}{
>{\centering\arraybackslash}m{0.5cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{0.5cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
\hline
\multicolumn{12}{c}{\textbf{unseen categories, without occlusions}}\\
\hline
\\[-0.2cm]
\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Bottle}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_41_0_10/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_41_0_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_41_0_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_41_0_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_41_0_10/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_53_3_9/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_53_3_9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_53_3_9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_53_3_9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bottle_53_3_9/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Bus}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_5_2_12/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_5_2_12/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_5_2_12/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_5_2_12/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_5_2_12/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_79_3_13/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_79_3_13/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_79_3_13/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_79_3_13/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/bus_79_3_13/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Clock}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_43_0_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_43_0_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_43_0_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_43_0_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_43_0_8/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_52_2_12/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_52_2_12/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_52_2_12/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_52_2_12/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/clock_52_2_12/proba.png}}\\


\parbox[t]{0mm}{\rotatebox[origin=l]{90}{Dishwasher}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_18_0_4/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_18_0_4/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_18_0_4/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_18_0_4/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_18_0_4/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_19_4_2/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_19_4_2/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_19_4_2/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_19_4_2/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/dishwasher_19_4_2/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Guitar}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_38_7_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_38_7_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_38_7_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_38_7_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_38_7_8/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_55_4_13/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_55_4_13/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_55_4_13/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_55_4_13/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/guitar_55_4_13/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Mug}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_16_4_11/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_16_4_11/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_16_4_11/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_16_4_11/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_16_4_11/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_37_7_1/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_37_7_1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_37_7_1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_37_7_1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/mug_37_7_1/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Pistol}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_20_0_3/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_20_0_3/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_20_0_3/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_20_0_3/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_20_0_3/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_21_2_9/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_21_2_9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_21_2_9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_21_2_9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/pistol_21_2_9/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=l]{90}{Skateboard}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_3_6_3/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_3_6_3/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_3_6_3/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_3_6_3/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_3_6_3/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_14_2_5/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_14_2_5/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_14_2_5/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_14_2_5/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/skateboard_14_2_5/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=c]{90}{Train}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_9__15/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_9__15/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_9__15/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_9__15/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_9__15/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_46__6/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_46__6/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_46__6/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_46__6/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/train_46__6/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=c]{90}{Washer}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_12_2_12/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_12_2_12/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_12_2_12/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_12_2_12/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_12_2_12/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_69_5_9/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_69_5_9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_69_5_9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_69_5_9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary/washer_69_5_9/proba.png}}\\

&Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution & &Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution\\
\end{tabular}
\end{tabular}
}
% \vspace{3mm}
\caption{\label{fig:resultsNoOcclusion} {\bf Visual results on unseen categories from ShapeNet, without occlusions}. The arrow indicates the pose with the highest probability as recovered by our method. We visually compare to PIZZA, which is the method with the second best performance. \textbf{We visualize the predicted poses by rendering the object from these poses, but the 3D model is only used for visualization purposes, not as input to our method. Similarly, we use the canonical pose of the 3D model to visualize this distribution, but not as input to our method.}
} 
\end{figure*}

==> sections/6_supp_qualitative_occlusion.tex <==
\begin{figure*}
% \newlength{\imageheight}
\setlength\imageheight{1.50cm}
\centering
\setlength\lineskip{3.pt}
\setlength\tabcolsep{2.pt} 
{\small
\begin{tabular}{c}
\begin{tabular}{
>{\centering\arraybackslash}m{0.5cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{0.5cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
\hline
\multicolumn{12}{c}{\textbf{unseen categories, with occlusions}}\\
\hline
\\[-0.2cm]
\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Bottle}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_11_1_6/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_11_1_6/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_11_1_6/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_11_1_6/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_11_1_6/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_41_0_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_41_0_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_41_0_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_41_0_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bottle_41_0_8/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Bus}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_10_7_11/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_10_7_11/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_10_7_11/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_10_7_11/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_10_7_11/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_74_5_10/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_74_5_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_74_5_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_74_5_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/bus_74_5_10/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Clock}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_7_6_9/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_7_6_9/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_7_6_9/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_7_6_9/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_7_6_9/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_22_7_5/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_22_7_5/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_22_7_5/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_22_7_5/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/clock_22_7_5/proba.png}}\\


\parbox[t]{0mm}{\rotatebox[origin=l]{90}{Dishwasher}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_18_0_3/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_18_0_3/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_18_0_3/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_18_0_3/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_18_0_3/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_25_6_2/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_25_6_2/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_25_6_2/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_25_6_2/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/dishwasher_25_6_2/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Guitar}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_26_0_1/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_26_0_1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_26_0_1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_26_0_1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_26_0_1/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_27_1_7/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_27_1_7/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_27_1_7/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_27_1_7/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/guitar_27_1_7/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Mug}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_17_0_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_17_0_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_17_0_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_17_0_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_17_0_8/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_56_2_2/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_56_2_2/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_56_2_2/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_56_2_2/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/mug_56_2_2/proba.png}}\\

\parbox[t]{0mm}{\rotatebox[origin=c]{90}{Pistol}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_0_3_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_0_3_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_0_3_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_0_3_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_0_3_8/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_2_4_10/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_2_4_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_2_4_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_2_4_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/pistol_2_4_10/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=l]{90}{Skateboard}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_32_0_3/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_32_0_3/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_32_0_3/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_32_0_3/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_32_0_3/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_14_2_8/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_14_2_8/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_14_2_8/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_14_2_8/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/skateboard_14_2_8/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=c]{90}{Train}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_29__1/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_29__1/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_29__1/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_29__1/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_29__1/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_51__7/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_51__7/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_51__7/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_51__7/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/train_51__7/proba.png}}\\

\parbox[t]{1mm}{\rotatebox[origin=c]{90}{Washer}} & \frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_59_1_10/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_59_1_10/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_59_1_10/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_59_1_10/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_59_1_10/proba.png}}&
&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_64_3_6/ref.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_64_3_6/1_query_crop.png}} &
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_64_3_6/pizza.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_64_3_6/0_pred_crop.png}}&
\frame{\includegraphics[height=\imageheight, ]{figures/supplementary_occlusion/washer_64_3_6/proba.png}}\\

&Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution & &Reference  & Query & PIZZA~\cite{nguyen_pizza_2022} & Ours & Pose distribution\\
\end{tabular}
\end{tabular}
}
\vspace{-5pt}
\caption{\label{fig:resultsOcclusion} {\bf Visual results on unseen categories from ShapeNet, with occlusions}. The arrow indicates the pose with the highest probability as recovered by our method. We visually compare with PIZZA, which is the method with the second best performance. \textbf{We visualize the predicted poses by rendering the object from these poses, but the 3D model is only used for visualization purposes, not as input to our method. Similarly, we use the canonical pose of the 3D model to visualize this distribution, but not as input to our method.}
} 
\end{figure*}

==> tables/shapeNet_std.tex <==
\begin{table*}[!b]
\addtolength{\tabcolsep}{1pt}
\centering
    \scalebox{.65}{
    \begin{tabular}{@{}l l | ccccccccccc | c@{}}
	\toprule
	& Method &  novel inst. & bottle$^*$ & bus & clock & dishwasher & guitar & mug & pistol & skateboard & train & washer & mean \\
	\midrule
	\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{$\bm{\AccThirty}\uparrow$}}} 
	& ViewNet \cite{mariotti_viewnet_2021} & {\bf 77.5} $\pm$ 4.2 &  48.4 $\pm$ 2.4 &  36.2 $\pm$ 4.8 &  23.5 $\pm$ 3.1 &  16.4 $\pm$ 4.1 &  37.8 $\pm$ 8.1 &  31.3 $\pm$ 5.2 &  17.9 $\pm$ 4.1 &  33.9 $\pm$ 4.8 &  44.8 $\pm$ 4.1 &  25.1 $\pm$ 4.8 &  35.7 $\pm$ 4.4  \\
	& SSVE \cite{mariotti_semi-supervised_2020} & 75.3 $\pm$ 3.2 &  61.5 $\pm$ 2.2 &  38.2 $\pm$ 3.7 &  41.8 $\pm$ 3.1 &  21.3 $\pm$ 2.9 &  46.8 $\pm$ 8.7 &  38.4 $\pm$ 4.6 &  36.8 $\pm$ 3.6 & {\bf 62.3} $\pm$ 4.1 &  41.5 $\pm$ 3.5 &  50.8 $\pm$ 3.5 &  46.8 $\pm$ 4.6  \\
	& PIZZA \cite{nguyen_pizza_2022} &  72.3 $\pm$ 3.5 &  76.0 $\pm$ 2.8 &  38.6 $\pm$ 5.1 &  38.5 $\pm$ 2.7 &  32.6 $\pm$ 5.1 &  30.8 $\pm$ 8.6 &  35.6 $\pm$ 4.2 &  40.4 $\pm$ 2.3 &  58.3 $\pm$ 3.1 &  52.9 $\pm$ 5.1 &  {\bf 61.0} $\pm$ 4.6 &  48.8 $\pm$ 3.8 \\
	& 3DiM \cite{3dim} & 77.3 $\pm$ 2.1 &  95.1 $\pm$ 1.9 &  43.5 $\pm$ 4.1 &  23.6 $\pm$ 3.2 &  24.5 $\pm$ 2.6 &  36.0 $\pm$ 5.3 &  32.0 $\pm$ 3.1 &  31.9 $\pm$ 2.5 &  50.3 $\pm$ 3.5 &  37.0 $\pm$ 3.2 &  56.1 $\pm$ 2.9 &  46.1 $\pm$ 3.6	\\
	
	& Ours (top 1) & 75.5 $\pm$ 1.3 &  {\bf 96.0 } $\pm$ 1.1 &  {\bf 53.6} $\pm$ 3.2 &  {\bf 48.0} $\pm$ 2.1 &  {\bf 48.0} $\pm$ 1.8 &  {\bf 49.0} $\pm$ 5.1 &  {\bf 44.6} $\pm$ 2.3 &  {\bf 69.0} $\pm$ 3.1 &  57.8 $\pm$ 2.8 &  {\bf 55.2} $\pm$ 2.3 &  60.6 $\pm$ 2.0 &  {\bf  59.8} $\pm$ 3.1 \\
	\cmidrule{2-14}
	& Ours (top 3) & 92.0 $\pm$ 1.5 & 97.4 $\pm$ 0.9 & 83.8 $\pm$ 2.5 & 73.4 $\pm$ 3.6 & 78.5 $\pm$ 2.2 & 66.8 $\pm$ 4.5 & 56.0 $\pm$ 2.0 & 83.8 $\pm$ 3.1 & 86.2 $\pm$ 2.2 & 86.0 $\pm$ 1.9 & 84.4 $\pm$ 2.0 & 80.8 $\pm$ 2.1 \\
	& Ours (top 5) & 95.5 $\pm$ 0.8 & 97.8 $\pm$ 0.2 & 89.8 $\pm$ 2.0 & 80.4 $\pm$ 3.0 & 88.2 $\pm$ 2.0 & 74.6 $\pm$ 4.6 & 62.8 $\pm$ 2.1 & 88.4 $\pm$ 2.6 & 92.8 $\pm$ 2.0 & 95.4 $\pm$ 1.7 & 93.4 $\pm$ 2.1 & 87.1 $\pm$ 1.7 \\
    \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{$\bm{\MedErr}\downarrow$}}}  & ViewNet \cite{mariotti_viewnet_2021} &  6.6 $\pm$ 5.0 & 26.7 $\pm$ 3.5 & 35.8 $\pm$ 5.1 & 40.3 $\pm$ 4.6 & 96.3 $\pm$ 3.0 & 50.6 $\pm$ 6.9 & 51.6 $\pm$ 4.1 & 42.8 $\pm$ 4.1 & 37.4 $\pm$ 3.7 & 26.8 $\pm$ 3.1 & 44.3 $\pm$ 2.9 & 41.7 $\pm$ 4.9 \\
    & SSVE \cite{mariotti_semi-supervised_2020} & 6.1 $\pm$ 3.1 & 23.8 $\pm$ 2.6 & 45.2 $\pm$ 3.0 & 41.9 $\pm$ 3.3 & 90.4 $\pm$ 2.3 & 47.6 $\pm$ 7.6 & 49.6 $\pm$ 4.1 & 24.0 $\pm$ 2.9 &  13.5 $\pm$ 3.8 & 24.9 $\pm$ 4.1 & 48.1 $\pm$ 3.8 & 37.7 $\pm$ 4.2\\
    & PIZZA     \cite{nguyen_pizza_2022} &5.8 $\pm$ 2.6 & 25.5 $\pm$ 3.4 & 26.4 $\pm$ 4.1 & 43.2 $\pm$ 4.1 & 80.6 $\pm$ 2.7 & 40.2 $\pm$ 5.1 & 45.5 $\pm$ 4.5 & 23.4 $\pm$ 2.1 & 17.3 $\pm$ 3.1 & 20.3 $\pm$ 5.1 & 38.5 $\pm$ 5.1 & 33.3 $\pm$ 4.7
 \\
    & 3DiM \cite{3dim} & {\bf 5.7} $\pm$ 3.1 & {\bf 1.8} $\pm$ 2.4 & 19.8 $\pm$ 3.5 & 47.3 $\pm$ 3.7 & 98.8 $\pm$ 2.9 & 35.2 $\pm$ 5.8 & 35.7 $\pm$ 2.5 & 21.2 $\pm$ 2.8 & {\bf 12.5} $\pm$ 2.9 & {\bf 17.6} $\pm$ 2.5 & 19.2 $\pm$ 2.6 & 28.6 $\pm$ 3.0 \\
	& Ours (top 1) & 8.1 $\pm$ 1.3 & {\bf 1.8} $\pm$ 1.1 & {\bf 18.4} $\pm$ 3.2 & {\bf 39.9} $\pm$ 2.1 & {\bf 77.6} $\pm$ 1.8 & {\bf 31.6} $\pm$ 5.1 & {\bf 35.5} $\pm$ 2.3 & {\bf 13.4} $\pm$ 3.1 & 15.5 $\pm$ 2.8 & 18.3 $\pm$ 2.3 & {\bf 8.5} $\pm$ 2.0 & {\bf 24.4} $\pm$ 3.1\\
	\cmidrule{2-14}
	& Ours (top 3) & 5.0 $\pm$ 1.0 & 1.3 $\pm$ 0.7 & 5.8 $\pm$ 3.6 & 9.1 $\pm$ 2.1 & 4.8 $\pm$ 2.2 & 16.0 $\pm$ 4.1 & 22.6 $\pm$ 3.1 & 8.1 $\pm$ 1.8 & 6.5 $\pm$ 1.6 & 6.7 $\pm$ 2.6 & 5.7 $\pm$ 2.6 & 8.3 $\pm$ 2.4\\
	& Ours (top 5) & 4.5 $\pm$ 0.8 & 1.2 $\pm$ 0.6 & 4.5 $\pm$ 3.0 & 7.1 $\pm$ 2.0 & 4.4 $\pm$ 2.1 & 11.6 $\pm$ 3.1 & 18.4 $\pm$ 2.6 & 6.1 $\pm$ 2.4 & 5.6 $\pm$ 1.7 & 4.9 $\pm$ 2.0 & 5.0 $\pm$ 2.8 & 6.6 $\pm$ 2.1\\
	\bottomrule
	\end{tabular}
    }
    % \vspace*{-5mm}
    \caption{{\bf Quantitative results on ShapeNet dataset.} We treat “bottle" as a symmetric category, i.e., the error is only the difference of elevation angle. Since the quality of prediction may depend on the reference image, we report \nguyen{the average and the standard deviation} of 5 runs with 5 different reference images.  
    }
    % We provide the std of this score in the supplementary material. 
    
    %\nguyenrmk{Yes, it's time reason. And yes again, 'unseen ins.' corresponds to unseen instances of training categories. It's out of scope, I agree but since we re-implemented all these methods, it's important to show that it works correctly for seen categories so the reviews can know we re-implement them successfully.}
  \label{tab:resultStd}
  \end{table*} 
